The Impact of Hole Geometry on Relative Robustness of In-Painting Networks: An Empirical Study

In-painting networks use existing pixels to generate appropriate pixels to fill "holes" placed on parts of an image. A 2-D in-painting network's input usually consists of (1) a three-channel 2-D image, and (2) an additional channel for the "holes" to be in-painted in that image. In this paper, we study the robustness of a given in-painting neural network against variations in hole geometry distributions. We observe that the robustness of an in-painting network is dependent on the probability distribution function (PDF) of the hole geometry presented to it during its training even if the underlying image dataset used (in training and testing) does not alter. We develop an experimental methodology for testing and evaluating relative robustness of in-painting networks against four different kinds of hole geometry PDFs. We examine a number of hypothesis regarding (1) the natural bias of in-painting networks to the hole distribution used for their training, (2) the underlying dataset's ability to differentiate relative robustness as hole distributions vary in a train-test (cross-comparison) grid, and (3) the impact of the directional distribution of edges in the holes and in the image dataset. We present results for L1, PSNR and SSIM quality metrics and develop a specific measure of relative in-painting robustness to be used in cross-comparison grids based on these quality metrics. (One can incorporate other quality metrics in this relative measure.) The empirical work reported here is an initial step in a broader and deeper investigation of "filling the blank" neural networks' sensitivity, robustness and regularization with respect to hole "geometry" PDFs, and it suggests further research in this domain.

==> fragment_40MB.tex <==
\subsubsection{Using the 40 MB in-painting network} \label{results_40MB}

\textit{\textbf{TODO: FINISH This PLACE HOLDER --- Figure \ref{fig:pf_f64} is for 40MB.
}
}

\input{pf_f64}

\subsection{\textit{TODO:} Spurious and Hanging Material}

Nevertheless, the results in Figures \ref{fig:pf_means} and \ref{fig:pf_f32} also raise some other questions:

[TODO: FINISH THIS SECTION BY INCLUDING THE RESULTS for bigger networks or longer training. They may make no differnece] \textit{TODO: FINISH THIS SECTION.}

To answer the second question and discuss the third, we formalize our methodology in section \ref{relative-power}.

Reviewing the results in Figure \ref{fig:pf_f32} raises some additional questions: 

\begin{itemize}
\item Is there an effective way to combine the quality metrics to compare the power differentials when the same network is trained with varying hole distributions?
\item What is the best way to reveal the power differentials? Do datasets use have any impact? 
\item
How similar or different are the power of $R4$-trained and $RFOM$-trained networks?  
\end{itemize} 

The first question is answered with cross-comparisons like the one shown in \ref{fig:pf_f32}. In section \ref{relative-power}, we discuss a more ``holistic'' method to combine the quality metrics to compare power of networks. 


==> pf_means.tex <==
%%%%%%%%%%%%%%% means of metric values:
\begin{figure*}[h]
    \centering
    \subfigure[Mean L1, PSNR and SSIM comparisons (10MB model / MIT Places)]
    {
        \includegraphics[width=0.15\linewidth, trim=4 4 4 4,clip]
        {Places_f32_L1}
        \includegraphics[width=0.15\linewidth, trim=4 4 4 4,clip]
        {Places_f32_PSNR}
        \includegraphics[width=0.15\linewidth, trim=4 4 4 4,clip]
        {Places_f32_SSIM}
        \label{fig:P_f32m}
    } 
    \rulesep    
    \subfigure[Mean L1, PSNR and SSIM comparisons (10MB model / CUHK CelebA)]
    {
        \includegraphics[width=0.15\linewidth, trim=4 4 4 4,clip]
        {CelebA_f32_L1}
        \includegraphics[width=0.15\linewidth, trim=4 4 4 4,clip]
        {CelebA_f32_PSNR}
        \includegraphics[width=0.15\linewidth, trim=4 4 4 4,clip]
        {CelebA_f32_SSIM}
        \label{fig:F_f32m}
    } 
    \caption{Mean quality metrics on the test set. Left triplet: MIT Places. Right triplet: CUHK CelebA. Cross-comparison of training and test hole distribution schemes. Table \ref{tab:color_scheme} provides color code for training hole distribution. \textit{Direction of polar axis indicates test hole distribution:} \textit{0-degree} for $RFOM$, \textit{90-degree} for $RR$, \textit{180-degree} for $R4$, and \textit{270-degree} for $RGS$. Clearly, there would be more polar axis in this diagram if a greater number of hole distributions for cross comparison purposes are used. As such, normalized areas (or inverse of normalized areas, in the case of $L_1$) of polygons for each in-training hole distribution can also potentially be used to compare overall power of that so-trained network, for any of the given metrics.}
    \label{fig:pf_means}
\end{figure*}


%%%%%%%%%%%%%%% These 40 MB results should be held back.
%%%%%%%%%%%%%%% Instead wait to include the 40MB for CelebA
%    \\
%    \subfigure[Mean L1, PSNR and SSIM comparisons (40MB model / MIT Places)]
%    {
%        \includegraphics[width=0.3\linewidth, trim=4 4 4 4,clip]
%        {Places_f64_L1}
%        \includegraphics[width=0.3\linewidth, trim=4 4 4 4,clip]
%        {Places_f64_PSNR}
%        \includegraphics[width=0.3\linewidth, trim=4 4 4 4,clip]
%        {Places_f64_SSIM}
%    } \label{fig:P_f64m}


==> tex_fragments.tex <==
\begin{table*}
\begin{center}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
$Hole_trn$ & $Hole_tst$ & $l_1$ & $psnr$ & $ssim$ & $NN$ & $sch$ & $data_trn$ & $data_tst$ \\
\hline
\hline
$RandomRectangles$ & $RandomRectangles$ & \\
\hline
$RandomGeometricShapes$ & $RandomRectangles$ &  \\
\hline
$RandomizedFlowOcclusionMasks$ & $RandomRectangles$ &  \\
\hline % change test mode
$RandomRectangles$ & $RandomGeometricShapes$ & \\
\hline
$RandomGeometricShapes$ & $RandomGeometricShapes$ &  \\
\hline
$RandomizedFlowOcclusionMasks$ & $RandomGeometricShapes$ &  \\
\hline % chagne test mode
$RandomRectangles$ & $RandomizedFlowOcclusionMasks$ & \\
\hline
$RandomGeometricShapes$ & $RandomizedFlowOcclusionMasks$ &  \\
\hline
$RandomizedFlowOcclusionMasks$ & $RandomizedFlowOcclusionMasks$ &  \\
\hline
\hline %  change dataset
$RandomRectangles$ & $RandomRectangles$ & \\
\hline
$RandomGeometricShapes$ & $RandomRectangles$ &  \\
\hline
$RandomizedFlowOcclusionMasks$ & $RandomRectangles$ &  \\
\hline % change test mode
$RandomRectangles$ & $RandomGeometricShapes$ & \\
\hline
$RandomGeometricShapes$ & $RandomGeometricShapes$ &  \\
\hline
$RandomizedFlowOcclusionMasks$ & $RandomGeometricShapes$ &  \\
\hline % chagne test mode
$RandomRectangles$ & $RandomizedFlowOcclusionMasks$ & \\
\hline
$RandomGeometricShapes$ & $RandomizedFlowOcclusionMasks$ &  \\
\hline
$RandomizedFlowOcclusionMasks$ & $RandomizedFlowOcclusionMasks$ &  \\
\hline
\hline
\end{tabular}
\end{center}
\caption{Impact of training and test hole distribution on mean value of in-painting networks' empirical quality metrics.}
\label{tab:metrics_mean_value}
\end{table*}

